Sparsity Moves Computation: How FFN Architecture Reshapes Attention in Small Transformers

Architectural choices inside the Transformer feedforward network (FFN) block do not merely affect the block itself; they reshape the computations learned by the rest of the model. We study this effect in one-layer Transformers trained on digit addition with carry, modular arithmetic, and histogram counting. Comparing dense FFNs, gated linear units (GLUs), mixture-of-experts (MoE), and MoE-GLUs, we find that sparse MoE routing can shift computation from FFN to attention, with the strongest ablation-visible effect on carry-based addition. We decompose this redistribution into reduced per-token FFN capacity and sparse partitioning across experts. Critically, frozen random routing nearly matches learned routing, suggesting that redistribution is driven largely by architectural sparsity rather than router-learned specialization. As a secondary finding, GLU-style multiplicative gating rotates task-relevant Fourier structure out of the per-neuron basis and into distributed subspaces, making neuron-level interpretability less informative while preserving structured computation. We validate these conclusions with random-routing, narrow-FFN, and top-2 MoE controls, plus parameter-matching, activation-function, and width-scaling analyses. Together, these results show that local FFN design choices can have nonlocal consequences for Transformer computation.

==> results/attn_moves.tex <==

\label{sec:redistribution}

We begin with our central finding: replacing a dense FFN with a
Mixture-of-Experts layer fundamentally changes \emph{where} computation
happens in the transformer. We measure this via component ablation (zeroing
the output of attention or FFN at inference time) across three tasks of
varying complexity.

%% --- Figure 1: Component ablation (add-7 + modadd) ---
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/add-7/MoE_redistributes_computation/ablation_+7_5_seeds.png}
    \caption{Add-7 (3-digit, no norm). MoE retains 55.4\% accuracy without
    FFN, compared to 9.5\% for dense FFN and 20.9\% for GLU.}
    \label{fig:ablation-add7-total}
  \end{subfigure}
  \vspace{0.5em}
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/mod-add/MoE_redistributes_computation/ablation_modular_addition_5_seeds.png}
    \caption{Modular addition ($\mathbb{Z}_{113}$, no norm). MoE retains
    16.5\% without FFN vs.\ 1.5\% for dense FFN. The redistribution effect
    persists but is attenuated because modular addition requires nonlinear
    Fourier computation that attention cannot absorb.}
    \label{fig:ablation-modadd-total}
  \end{subfigure}
  \caption{\textbf{Component ablation across tasks} (5 seeds each).
  Exact-match accuracy under three conditions: normal (all components
  active), no attention (attention output zeroed), and no FFN (FFN output
  zeroed). MoE consistently retains more accuracy without FFN than dense
  variants, indicating that MoE's attention has learned to handle a
  substantial portion of the computation independently. The effect scales
  with task simplicity: +46\,pp on add-7 vs.\ +15\,pp on modular addition.}
  \label{fig:component-ablation}
\end{figure}

%% --- Figure 2: Per-position ablation + carry length ---
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/add-7/MoE_redistributes_computation/fig10_per_position_ablation.png}
    \caption{Per-position accuracy. \textbf{Left}: without FFN, MoE's
    attention handles later positions (hundreds, overflow) at 60--90\%
    accuracy, while dense FFN collapses to ${\sim}0\%$. \textbf{Right}:
    without attention, the pattern reverses. Dense FFN reaches
    ${\sim}100\%$ at later positions, while MoE's FFN only reaches
    ${\sim}50\%$ because it offloaded that work to attention during
    training.}
    \label{fig:per-position-ablation}
  \end{subfigure}
  \vspace{0.5em}
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/add-7/MoE_redistributes_computation/fig_ablation_by_carry.png}
    \caption{Ablation stratified by carry-chain length. The MoE advantage
    under no-FFN ablation holds across all carry lengths. Error bars at
    $L{=}2$ are large due to limited samples (63 of 1000 test numbers).}
    \label{fig:ablation-by-carry}
  \end{subfigure}
  \caption{\textbf{Position-dependent redistribution on add-7} (no norm, 5
  seeds). Later output positions require cross-position information to
  determine whether a carry arrived, which is what attention computes. MoE's
  routing bottleneck forced attention to learn this routing during training,
  producing a clean division of labor: attention handles positions where
  carry information must be routed, while FFN handles the local arithmetic.
  This division holds across carry-chain lengths.}
  \label{fig:position-redistribution}
\end{figure}

%% --- Figure 3: DLA cross-task comparison ---
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{images/mod-add/dla/fig_dla_cross_task.png}
  \caption{\textbf{Direct logit attribution across tasks} (no norm, 5
  seeds). Each bar shows the fraction of the correct output logit
  attributable to attention (red) vs.\ FFN (blue), measured by projecting
  each component's residual-stream contribution through the unembedding
  matrix. \textbf{(a)}~On modular addition, FFN dominates for all variants
  (88--99\%), with MoE's attention contributing only ${\sim}11\%$.
  \textbf{(b)}~On add-7, MoE's attention contributes ${\sim}60\%$ of the
  correct logit vs.\ ${\sim}40\%$ for dense FFN. Redistribution scales
  with task simplicity: it occurs when the computation is within attention's
  expressive capacity.}
  \label{fig:dla-cross-task}
\end{figure}

\paragraph{The redistribution effect.}
With FFN zeroed, MoE retains 55.4\% accuracy on add-7, compared to 9.5\%
for dense FFN and 20.9\% for GLU
(Figure~\ref{fig:ablation-add7-total}). This is not an inference-time
artifact but a \emph{training-time} effect: MoE's routing bottleneck
reduces effective per-token FFN capacity to ${\sim}1/E$, pressuring
attention to develop more structured circuits. We observe this directly:
MoE attention heads show cleaner functional specialization (digit-copying,
carry-sensitive context) than dense variants, and direct logit attribution
confirms attention contributes ${\sim}60\%$ of correct logits in MoE vs.\
${\sim}40\%$ in FFN even before any ablation
(Figure~\ref{fig:dla-cross-task}b).

\paragraph{Position-dependent redistribution.}
The effect is not uniform across output positions
(Figure~\ref{fig:per-position-ablation}). Later positions (tens, hundreds,
overflow) require cross-position information to determine whether a carry
arrived, which is precisely what attention computes. MoE's routing bottleneck
forced attention to learn this cross-position routing during training:
without FFN, MoE's attention reaches ${\sim}90\%$ at overflow and
${\sim}60\%$ at hundreds, while dense FFN's attention collapses to
${\sim}0\%$ because it never learned to route carry information.
Conversely, without attention, dense FFN reaches
${\sim}100\%$ at overflow while MoE's FFN only reaches ${\sim}50\%$,
having offloaded that work. The MoE advantage holds across all carry-chain
lengths (Figure~\ref{fig:ablation-by-carry}).

\paragraph{Expressiveness limits.}
Attention alone plateaus well below full accuracy for all variants;
the nonlinear interaction provided by FFN remains necessary for the complete
algorithm. Per-digit addition ($d \mapsto (d{+}k) \bmod 10$) is a linear
map, but multi-step carry propagation requires conjunctions ($d_0 \geq 3
\wedge d_1 = 9$) that attention cannot express: each head contributes an
additive term to the residual stream, yielding disjunctive rather than
conjunctive composition
\citep{Hahn2019TheoreticalLO, Merrill2021SaturatedTA}.

\paragraph{Cross-task validation.}
Modular addition requires a nonlinear algorithm (Fourier components over
$\mathbb{Z}_{113}$; \citealt{nanda2023progress}). Accordingly, no-FFN
accuracy is low for \emph{all} variants (MoE: 16.5\%, FFN: 1.5\%), but MoE
still retains ${10\times}$ more. The redistribution occurs, but it cannot
fully compensate when the FFN computation is irreducibly nonlinear
(Figure~\ref{fig:ablation-modadd-total}). Direct logit attribution confirms
this quantitatively: on modular addition, FFN accounts for 88--99\% of the
correct logit across all variants, whereas on add-7 MoE's attention
contributes the majority (Figure~\ref{fig:dla-cross-task}). On histogram
counting, redistribution is minimal (+0.7\,pp).
\citet{Behrens2024CountingIS} show that counting requires tight coupling
between attention (token mixing) and FFN (feature extraction), with the
feasible strategy depending on softmax normalization and FFN width.
\citet{Ouellette2023CountingAA} further demonstrate that softmax normalizes
away count magnitude (attention produces $\frac{1}{N}\sum c_i$ rather than
$\sum c_i$), making FFN essential for recovering absolute counts. Unlike
add-7, where per-digit operations are within attention's expressive capacity,
counting requires both components in a way that leaves no room for
redistribution.

\paragraph{Weight norm evidence.}
Weight norms confirm the mechanism: MoE compresses total weight norms
$0.63{\times}$ while GLU collapses FFN norms to $0.21{\times}$. Capacity is
being \emph{moved}, not added (Figure~\ref{fig:weight-norms}).


==> section_4_1_attention_moves.tex <==
% Section 4.1: MoE Redistributes Computation from FFN to Attention
% ----------------------------------------------------------------

\subsection{MoE Redistributes Computation from FFN to Attention}
\label{sec:redistribution}

We begin with our central finding: replacing a dense FFN with a
Mixture-of-Experts layer fundamentally changes \emph{where} computation
happens in the transformer. We measure this via component ablation (zeroing
the output of attention or FFN at inference time) across three tasks of
varying complexity.

%% --- Figure 1: Overall ablation on add-7 ---
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{images/add-7/MoE_redistributes_computation/ablation_+7_5_seeds.png}
  \caption{\textbf{Component ablation on add-7} (no norm, 5 seeds).
  Exact-match accuracy under three conditions: normal (all components
  active), no attention (attention output zeroed), and no FFN (FFN output
  zeroed). MoE retains 55.4\% accuracy without FFN, compared to 9.5\% for
  dense FFN and 20.9\% for GLU, indicating that MoE's attention has learned
  to handle a substantial portion of the computation independently.}
  \label{fig:ablation-add7-total}
\end{figure}

%% --- Figure 2: Per-position ablation on add-7 ---
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{images/add-7/MoE_redistributes_computation/fig10_per_position_ablation.png}
  \caption{\textbf{Per-position accuracy under component ablation} (add-7,
  no norm, 5 seeds). \textbf{(a)}~Without FFN: MoE's attention handles
  later output positions (hundreds, overflow) at 60--90\% accuracy, while
  dense FFN's attention collapses to ${\sim}0\%$ at those positions.
  \textbf{(b)}~Without attention: the pattern reverses. Dense FFN reaches
  ${\sim}100\%$ at later positions using FFN alone, while MoE's FFN only
  reaches ${\sim}50\%$ because it offloaded that work to attention during
  training. Later positions require cross-position carry information, which
  is precisely what attention computes.}
  \label{fig:per-position-ablation}
\end{figure}

%% --- Figure 3: Ablation by carry length on add-7 ---
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{images/add-7/MoE_redistributes_computation/fig_ablation_by_carry.png}
  \caption{\textbf{Component ablation stratified by carry-chain length}
  (add-7, no norm, 5 seeds). The MoE advantage under no-FFN ablation holds
  across all carry lengths. Error bars at $L{=}2$ are large due to limited
  samples (63 of 1000 test numbers, 6.3\%).}
  \label{fig:ablation-by-carry}
\end{figure}

%% --- Figure 4: Overall ablation on modular addition ---
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{images/mod-add/MoE_redistributes_computation/ablation_modular_addition_5_seeds.png}
  \caption{\textbf{Component ablation on modular addition} (no norm, 5
  seeds). The redistribution effect persists but is attenuated. MoE retains
  16.5\% without FFN vs.\ 1.5\% for dense FFN. Modular addition requires
  nonlinear Fourier computation that attention cannot absorb, limiting the
  degree of redistribution compared to add-7.}
  \label{fig:ablation-modadd-total}
\end{figure}

%% --- Figure 5: DLA cross-task comparison ---
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{images/dla/fig_dla_cross_task.png}
  \caption{\textbf{Direct logit attribution across tasks} (no norm, 5
  seeds). Each bar shows the fraction of the correct output logit
  attributable to attention (red) vs.\ FFN (blue), measured by projecting
  each component's residual-stream contribution through the unembedding
  matrix. \textbf{(a)}~On modular addition, FFN dominates for all variants
  (88--99\%), with MoE's attention contributing only ${\sim}11\%$.
  \textbf{(b)}~On add-7, MoE's attention contributes ${\sim}60\%$ of the
  correct logit vs.\ ${\sim}40\%$ for dense FFN. The contrast confirms that
  redistribution scales with task simplicity: it occurs when the computation
  is within attention's expressive capacity.}
  \label{fig:dla-cross-task}
\end{figure}

\paragraph{The redistribution effect.}
With FFN zeroed, MoE retains 55.4\% accuracy on add-7, compared to 9.5\%
for dense FFN and 20.9\% for GLU
(Figure~\ref{fig:ablation-add7-total}). This is not an inference-time
artifact but a \emph{training-time} effect: MoE's routing bottleneck
reduces effective per-token FFN capacity to ${\sim}1/E$, pressuring
attention to develop more structured circuits. We observe this directly:
MoE attention heads show cleaner functional specialization (digit-copying,
carry-sensitive context) than dense variants, and direct logit attribution
confirms attention contributes ${\sim}60\%$ of correct logits in MoE vs.\
${\sim}40\%$ in FFN even before any ablation
(Figure~\ref{fig:dla-cross-task}b).

\paragraph{Position-dependent redistribution.}
The effect is not uniform across output positions
(Figure~\ref{fig:per-position-ablation}). Later positions (tens, hundreds,
overflow) require cross-position information to determine whether a carry
arrived, which is precisely what attention computes. MoE's routing bottleneck
forced attention to learn this cross-position routing during training:
without FFN, MoE's attention reaches ${\sim}90\%$ at overflow and
${\sim}60\%$ at hundreds, while dense FFN's attention collapses to
${\sim}0\%$ because it never learned to route carry information.
Conversely, without attention, dense FFN reaches
${\sim}100\%$ at overflow while MoE's FFN only reaches ${\sim}50\%$,
having offloaded that work. The MoE advantage holds across all carry-chain
lengths (Figure~\ref{fig:ablation-by-carry}).

\paragraph{Expressiveness limits.}
Attention alone plateaus well below full accuracy for all variants;
the nonlinear interaction provided by FFN remains necessary for the complete
algorithm. Per-digit addition ($d \mapsto (d{+}k) \bmod 10$) is a linear
map, but multi-step carry propagation requires conjunctions ($d_0 \geq 3
\wedge d_1 = 9$) that attention cannot express: each head contributes an
additive term to the residual stream, yielding disjunctive rather than
conjunctive composition
\citep{Hahn2019TheoreticalLO, Merrill2021SaturatedTA}.

\paragraph{Cross-task validation.}
Modular addition requires a nonlinear algorithm (Fourier components over
$\mathbb{Z}_{113}$; \citealt{nanda2023progress}). Accordingly, no-FFN
accuracy is low for \emph{all} variants (MoE: 16.5\%, FFN: 1.5\%), but MoE
still retains ${10\times}$ more. The redistribution occurs, but it cannot
fully compensate when the FFN computation is irreducibly nonlinear
(Figure~\ref{fig:ablation-modadd-total}). Direct logit attribution confirms
this quantitatively: on modular addition, FFN accounts for 88--99\% of the
correct logit across all variants, whereas on add-7 MoE's attention
contributes the majority (Figure~\ref{fig:dla-cross-task}). On histogram
counting, redistribution is minimal (+0.7\,pp).
\citet{Behrens2024CountingIS} show that counting requires tight coupling
between attention (token mixing) and FFN (feature extraction), with the
feasible strategy depending on softmax normalization and FFN width.
\citet{Ouellette2023CountingAA} further demonstrate that softmax normalizes
away count magnitude (attention produces $\frac{1}{N}\sum c_i$ rather than
$\sum c_i$), making FFN essential for recovering absolute counts. Unlike
add-7, where per-digit operations are within attention's expressive capacity,
counting requires both components in a way that leaves no room for
redistribution.

\paragraph{Weight norm evidence.}
Weight norms confirm the mechanism: MoE compresses total weight norms
$0.63{\times}$ while GLU collapses FFN norms to $0.21{\times}$. Capacity is
being \emph{moved}, not added (Figure~\ref{fig:weight-norms}).

